Persistent Evidence of Local Image Properties in Generic ConvNets

Supervised training of a convolutional network for object classification should make explicit any information related to the class of objects and disregard any auxiliary information associated with the capture of the image or the variation within the object class. Does this happen in practice? Although this seems to pertain to the very final layers in the network, if we look at earlier layers we find that this is not the case. Surprisingly, strong spatial information is implicit. This paper addresses this, in particular, exploiting the image representation at the first fully connected layer, i.e. the global image descriptor which has been recently shown to be most effective in a range of visual recognition tasks. We empirically demonstrate evidences for the finding in the contexts of four different tasks: 2d landmark detection, 2d object keypoints prediction, estimation of the RGB values of input image, and recovery of semantic label of each pixel. We base our investigation on a simple framework with ridge rigression commonly across these tasks, and show results which all support our insight. Such spatial information can be used for computing correspondence of landmarks to a good accuracy, but should potentially be useful for improving the training of the convolutional nets for classification purposes.

==> Introduction_option.tex <==
\section{Introduction}

There is at least one alchemy associated with deep \CNNs. It
occurs when $\sim$100,000 iterations of SGD, in tandem with
$~1$million labelled training images from ImageNet, transform the
$\sim 40$ million randomly initialized weights of a deep \CNN{} into
the best, by a huge margin, performing known visual image classifier
\cite{}(many citations).
Alongside this high-level alchemy is another related one
w.r.t. the image representations learnt by the fully connected layers
of a deep \CNN, in particular, the first fully connected layers
\cite{}(a few citations). These representations are explicitly trained to retain
information relevant to semantic class.
The thrust of this paper is that we *show* they also retain {\em spatial}
information, including the location of object parts and keypoints of object. 

Existing studies presented some ideas of extracting spatial information
from an image with deep ConvNet: 
some trained a specialized ConvNet on spatial information and expected
the network to predict what has been trained to do (cite Deep pose, PANDA, Fergus's depth paper, etc...).
some others used a sliding window and compared the response of different
windows to localize the interesting properties (cite Overfeat, Berekly's paper, etc...).
%
Unlike existing approaches we show a generic ConvNet trained on ImageNet
is capable of predicting spatial information. In this respect, more recent work
have addressed \cite{BerkeleyNips14,BroxArxiv14} that it is possible to
recognize keypoints using a \CNN{} representation, but they only
consider representations extracted from convolutional layers
describing a subset of the image's subpatches.
% In this paper, we don't use sliding windows and use linear regression function over
Instead, we exploit the response of the first fully connected network and demonstrate
that it is useful to estimate spatial information of *various forms*.
% facial landmarks, object key-points, semantic segmentation as well as RGB reconstruction.
 

Why do we concentrate on the fully connected layers?  Prior work has
shown that these layers correspond to the most generic and compact
image representation and produce the best results, when combined with
a simple linear classifier, in a range of visual recognition tasks \cite{}.
%(Where best takes into consideration hand-crafted features such as SIFT and the representations extracted from the convolutional layers.)
Therefore the starting point of this work was to
examine what other information, besides visual semantic information,
is encoded and easily accessible from these representations.
 

In particular we show that one can learn a linear regression
function (with varying degrees of success) from a generic \CNN{}
representation extracted from a fully connected layer of an image to
facial landmarks, object key-points, semantic segmentation as well as RGB
values. 
We chose this fashion of the experiments to show the baseline of reliable spatial information.
%
What's fascinating is that during the training, the network has never been explicitly constrained to learn spatial information. In fact, the network is trained to be invariant of spatial information such as locations and poses.
% yet they end up in the fully connected layers and even in a more organized way than the original RGB.

The contributions of the paper is:\\
-\\
-\\
-

\section{Insight}

To illuminate why we feel this is surprising
we now review how a \CNN{} converts an RGB image, via different image
representations, into a semantic label.

The weights of a \CNN's convolutional layers encode a very large
number of compositional patterns of appearance that occur in the
training images. Thus the multiple response maps output by a
convolutional layer indicate which appearance patterns occur in
different sub-patches of a fixed size in the original image. The size
of these sub-patches then increases as we progress through the
convolutional layers. When we come to the first fully-connected layer
the network must compress the set of response maps
(20$\times$20$\times$200 numbers) produced by the final convolutional
layer into a mere 4096 numbers. The compression performed seeks to
optimize the ability of the network's classification layer (with
potentially some more intermediary fully-connected layers) to produce
output with semantic labels as defined by the ImageNet classification
task.

 
The weights of the first fully connected layer are, in general, not
particularly sparse. Therefore the \textit{what} and \text{where}
explicitly encoded in the convolutional layers are aggregated, merged
and conflated into the output nodes of this first fully connected
layer. At this stage it is impossible to backtrack from these
responses to spatial locations in the image. But still we show it is
possible to predict from this global image descriptor, using linear
regressors, the spatial location of object parts and keypoints.



%% 1 or 2 sentence about the emerge of ConvNets in the computer vision in the past 2 years.\\
%% While everyone agrees that ConvNet representation is by far the best feature set for visual recognition (cite lot's of papers) we show that spatial information including 2D landmarks, object keypoints, semantic segmentation of the image and even RGB values of the image DO exist in a single 4096 dimensional representation of a generic ConvNet trained on ImageNet. \\
%% Previously there where two strong trend to extract spatial information from an image. Some trained a specialized ConvNet on spatial information and expect the network to predict what is has been trained to do (cite Deep pose, PANDA, Fergus's depth paper, etc...) and on the other hand some used a sliding window and compared the response of different windows to localize the interesting properties (cite Overfear, Berekly's paper, etc...).\\
%% Our approach is different from two trends in the sense that we show a generic ConvNet trained on ImageNet is capable of predicting spatial information. In this paper, we don't use sliding windows and use linear regression function over the response of the first fully connected network to estimate facial landmarks, object key-points, RGB reconstruction and Semantic segmentations of the image(see chapter ...).\\
%% What's fascinating is that during the training, the network has never been explicitly constrained to learn spatial information. In fact, the network is trained to be invariant of spatial information like locations and poses, yet they end up in the fully connected layers and even in a more organized way than the original RGB.\\
%% For this paper we used linear regression function and we didn't even model the binary relation between dependent linear regressors (for example to regress to X and Y coordinate of a landmark, two independent linear regressors was trained). We chose this fashion of the experiment to show the baseline of reliable spatial information. \\
%% In section \ref{sec:applications} we explain our method of estimating spatial information and show that these informations can be extracted from a generic ConvNets using a single representation. We also provide a simple trick to boost the performance and show the immense potential in ...\\ 
%% Counterintuitive as this observation is, we provide on argument -amongst many- that why this information should ended up in a more organized manner than RGB in the fully connected representation.\\


%% There is at least one alchemy associated with deep \CNNs. It
%% occurs when $\sim$100,000 iterations of SGD, in tandem with
%% $~1$million labelled training images from ImageNet, transform the
%% $\sim 40$ million randomly initialized weights of a deep \CNN{} into
%% the best, by a huge margin, performing known visual image classifier.
%% But alongside this high-level alchemy is another related one
%% w.r.t. the image representations learnt by the fully connected layers
%% of a deep \CNN. These representations are explicitly trained to retain
%% information relevant to semantic class, but in this paper we show they
%% also retain spatial information about the location of object parts and
%% keypoints of objects. To illuminate why we feel this is surprising
%% we now review how a \CNN{} converts an RGB image, via different image
%% representations, into a semantic label.

%% The weights of a \CNN's convolutional layers encode a very large
%% number of compositional patterns of appearance that occur in the
%% training images. Thus the multiple response maps output by a
%% convolutional layer indicate which appearance patterns occur in
%% different sub-patches of a fixed size in the original image. The size
%% of these sub-patches then increases as we progress through the
%% convolutional layers. When we come to the first fully-connected layer
%% the network must compress the set of response maps
%% (20$\times$20$\times$200 numbers) produced by the final convolutional
%% layer into a mere 4096 numbers. The compression performed seeks to
%% optimize the ability of the network's classification layer (with
%% potentially some more intermediary fully-connected layers) to produce
%% output with semantic labels as defined by the ImageNet classification
%% task.

%% The weights of the first fully connected layer are, in general, not
%% particularly sparse. Therefore the \textit{what} and \text{where}
%% explicitly encoded in the convolutional layers are aggregated, merged
%% and conflated into the output nodes of this first fully connected
%% layer. At this stage it is impossible to backtrack from these
%% responses to spatial locations in the image. But still we show it is
%% possible to predict from this global image descriptor, using linear
%% regressors, the spatial location of object parts and keypoints. Others
%% have shown \cite{BerkeleyNips14,BroxArxiv14} that it is possible to
%% recognize keypoints using a \CNN{} representation, but they only
%% consider representations extracted from convolutional layers
%% describing a subset of the image's subpatches.

%% Why do we concentrate on the fully connected layers?  Prior work has
%% shown that these layers correspond to the most generic and compact
%% image representation and produce the best results, when combined with
%% a simple linear classifier, in a range of visual recognition
%% tasks\cite{}. (Where best takes into consideration hand-crafted
%% features such as SIFT and the representations extracted from the
%% convolutional layers.) Therefore the starting point of this work was to
%% examine what other information, besides visual semantic information,
%% is encoded and easily accessible from these representations.



%% In particular we show that one can learn a linear regression
%% function (with varying degrees of success) from a generic \CNN{}
%% representation extracted from a fully connected layer of an image to
%% (SHOULD ADD MORE DETAIL ABOUT OUR CONCRETE RESULTS IN THIS list)
%%  \begin{enumerate}
%%  \item 2d facial landmarks (Section \ref{}),
%%  \item 2d body joints (Section \ref{}),
%%  \item 2d object keypoints (Section \ref{}),
%%  \item original RGB image (Section \ref{}),
%%  \item pose of an object (Section \ref{}).
%%  \end{enumerate}
%%  These results indicate that the following information is implicitly encoded
%%  in the \CNN{} representation
%%  \begin{itemize}
%%  \item spatial location of object parts
%%  \item rgb
%%  \item object pose
%%  \end{itemize}

%% We hope in future work to shed light on the hows and whys these
%% representations encode this information.  But the fear of
%% hallucinating experimental evidence for the elephant in the room - the
%% concept of \textit{disentanglement} - means that paper is devoted to
%% reporting our concrete but surprising results.

% gallimaufry

